Constrained existence problem for weak subgame perfect equilibria with omega-regular Boolean objectives (full version)

We study multiplayer turn-based games played on a finite directed graph such that each player aims at satisfying an omega-regular Boolean objective. Instead of the well-known notions of Nash equilibrium (NE) and subgame perfect equilibrium (SPE), we focus on the recent notion of weak subgame perfect equilibrium (weak SPE), a refinement of SPE. In this setting, players who deviate can only use the subclass of strategies that differ from the original one on a finite number of histories. We are interested in the constrained existence problem for weak SPEs. We provide a complete characterization of the computational complexity of this problem: it is P-complete for Explicit Muller objectives, NP-complete for Co-B\"uchi, Parity, Muller, Rabin, and Streett objectives, and PSPACE-complete for Reachability and Safety objectives (we only prove NP-membership for B\"uchi objectives). We also show that the constrained existence problem is fixed parameter tractable and is polynomial when the number of players is fixed. All these results are based on a fine analysis of a fixpoint algorithm that computes the set of possible payoff profiles underlying weak SPEs.

==> vl-ccl.tex <==
%!TEX root=main.tex
\section{Conclusion and future work}

\fbox{Blabla de conclusion}

\begin{itemize}
	\item complexité exacte pour Büchi
	\item fonction de gain qualitative -> fonction de gain quantitative
	\item weak SPE - > SPE
	\item l'étude du coût d'un chemin est un important pour le calcul de la complexité FPT mais cette étude pourrait être faite plus finement, en évitant de repasser par des jeux à deux joueurs.
	\item Est-ce qu'on parle de l'aspect algorithmique et des SCCs?
\end{itemize}





%\fbox{suite a mettre ailleurs}
%
%\begin{remark}
%	We discuss the conditions of those different properties.
%	\begin{enumerate}
%	\item The equivalence between (\ref{Lasse:1}) and (\ref{Lasse:2}) holds for a larger class of games than multiplayer Boolean games. It suffies that the gain functions $\Gain_i$ are prefix-independent and finite-range for all $i \in \Pi$.
%	\item In the same way, we can state the same kind of equivalence between (\ref{Lasse:2}) and (\ref{assert:existenceWitnesses}) if the gain functions $\Gain_i$ are prefix-independent and finite-range  for all $i \in \Pi$ and if we remove the condition on the form of the symbolic witnesses. They do not have to be lassoes and there is no bound on their length.
%	\item If we want a bound on the memory size required by the strategies of the equilibrium build in (\ref{assert:existenceWSPEpoly}), we only have to know the maximal memory needed to represent the symbolic witnesses in $\Wit$. Let $s$ be the size of this memory, if for all $i\in \Pi$ the gain functions $\Gain_i$ are prefix-independent and finite range, we can build a weak SPE with memory in $\mathcal{O}(|\Pi|\cdot|V|\cdot s)$.
%\end{enumerate}
%\end{remark}
%\todo[inline]{Vérifier que toutes ces affirmations sont bien vraies.}
